Amplitude analysis of the $B_{(s)} \to K^{*0} \overline{K}^{*0}$ decays and measurement of the branching fraction of the $B \to K^{*0} \overline{K}^{*0}$ decay

The $B^0 \to K^{*0} \overline{K}^{*0}$ and $B^0_s \to K^{*0} \overline{K}^{*0}$ decays are studied using proton-proton collision data corresponding to an integrated luminosity of 3fb$^{-1}$. An untagged and time-integrated amplitude analysis of $B^0_{(s)} \to (K^+\pi^-)(K^-\pi^+) $ decays in two-body invariant mass regions of 150 MeV$/c^2$ around the $K^{*0}$ mass is performed. A stronger longitudinal polarisation fraction in the ${B^0 \to K^{*0} \overline{K}^{*0}}$ decay, ${f_L = 0.724 \pm 0.051 \,({\rm stat}) \pm 0.016 \,({\rm syst})}$, is observed as compared to ${f_L = 0.240 \pm 0.031 \,({\rm stat}) \pm 0.025 \,({\rm syst})}$ in the ${B^0_s\to K^{*0} \overline{K}^{*0}}$ decay. The ratio of branching fractions of the two decays is measured and used to determine $\mathcal{B}(B^0 \to K^{*0} \overline{K}^{*0}) = (8.0 \pm 0.9 \,({\rm stat}) \pm 0.4 \,({\rm syst})) \times 10^{-7}$.

==> LHCb_Authorship_25-Jan-2019_arXiv.tex <==
LHCb Collaboration:
R. Aaij,
C. Abell{\'a}n Beteta,
B. Adeva,
M. Adinolfi,
C.A. Aidala,
Z. Ajaltouni,
S. Akar,
P. Albicocco,
J. Albrecht,
F. Alessio,
M. Alexander,
A. Alfonso Albero,
G. Alkhazov,
P. Alvarez Cartelle,
A.A. Alves Jr,
S. Amato,
Y. Amhis,
L. An,
L. Anderlini,
G. Andreassi,
M. Andreotti,
J.E. Andrews,
F. Archilli,
J. Arnau Romeu,
A. Artamonov,
M. Artuso,
K. Arzymatov,
E. Aslanides,
M. Atzeni,
B. Audurier,
S. Bachmann,
J.J. Back,
S. Baker,
V. Balagura,
W. Baldini,
A. Baranov,
R.J. Barlow,
S. Barsuk,
W. Barter,
M. Bartolini,
F. Baryshnikov,
V. Batozskaya,
B. Batsukh,
A. Battig,
V. Battista,
A. Bay,
F. Bedeschi,
I. Bediaga,
A. Beiter,
L.J. Bel,
S. Belin,
N. Beliy,
V. Bellee,
N. Belloli,
K. Belous,
I. Belyaev,
G. Bencivenni,
E. Ben-Haim,
S. Benson,
S. Beranek,
A. Berezhnoy,
R. Bernet,
D. Berninghoff,
E. Bertholet,
A. Bertolin,
C. Betancourt,
F. Betti,
M.O. Bettler,
Ia. Bezshyiko,
S. Bhasin,
J. Bhom,
M.S. Bieker,
S. Bifani,
P. Billoir,
A. Birnkraut,
A. Bizzeti,
M. Bj{\o}rn,
M.P. Blago,
T. Blake,
F. Blanc,
S. Blusk,
D. Bobulska,
V. Bocci,
O. Boente Garcia,
T. Boettcher,
A. Bondar,
N. Bondar,
S. Borghi,
M. Borisyak,
M. Borsato,
M. Boubdir,
T.J.V. Bowcock,
C. Bozzi,
S. Braun,
M. Brodski,
J. Brodzicka,
A. Brossa Gonzalo,
D. Brundu,
E. Buchanan,
A. Buonaura,
C. Burr,
A. Bursche,
J. Buytaert,
W. Byczynski,
S. Cadeddu,
H. Cai,
R. Calabrese,
R. Calladine,
M. Calvi,
M. Calvo Gomez,
A. Camboni,
P. Campana,
D.H. Campora Perez,
L. Capriotti,
A. Carbone,
G. Carboni,
R. Cardinale,
A. Cardini,
P. Carniti,
K. Carvalho Akiba,
G. Casse,
M. Cattaneo,
G. Cavallero,
R. Cenci,
M.G. Chapman,
M. Charles,
Ph. Charpentier,
G. Chatzikonstantinidis,
M. Chefdeville,
V. Chekalina,
C. Chen,
S. Chen,
S.-G. Chitic,
V. Chobanova,
M. Chrzaszcz,
A. Chubykin,
P. Ciambrone,
X. Cid Vidal,
G. Ciezarek,
F. Cindolo,
P.E.L. Clarke,
M. Clemencic,
H.V. Cliff,
J. Closier,
V. Coco,
J.A.B. Coelho,
J. Cogan,
E. Cogneras,
L. Cojocariu,
P. Collins,
T. Colombo,
A. Comerma-Montells,
A. Contu,
G. Coombs,
S. Coquereau,
G. Corti,
C.M. Costa Sobral,
B. Couturier,
G.A. Cowan,
D.C. Craik,
A. Crocombe,
M. Cruz Torres,
R. Currie,
C.L. Da Silva,
E. Dall'Occo,
J. Dalseno,
C. D'Ambrosio,
A. Danilina,
P. d'Argent,
A. Davis,
O. De Aguiar Francisco,
K. De Bruyn,
S. De Capua,
M. De Cian,
J.M. De Miranda,
L. De Paula,
M. De Serio,
P. De Simone,
J.A. de Vries,
C.T. Dean,
W. Dean,
D. Decamp,
L. Del Buono,
B. Delaney,
H.-P. Dembinski,
M. Demmer,
A. Dendek,
D. Derkach,
O. Deschamps,
F. Desse,
F. Dettori,
B. Dey,
A. Di Canto,
P. Di Nezza,
S. Didenko,
H. Dijkstra,
F. Dordei,
M. Dorigo,
A.C. dos Reis,
A. Dosil Su{\'a}rez,
L. Douglas,
A. Dovbnya,
K. Dreimanis,
L. Dufour,
G. Dujany,
P. Durante,
J.M. Durham,
D. Dutta,
R. Dzhelyadin,
M. Dziewiecki,
A. Dziurda,
A. Dzyuba,
S. Easo,
U. Egede,
V. Egorychev,
S. Eidelman,
S. Eisenhardt,
U. Eitschberger,
R. Ekelhof,
L. Eklund,
S. Ely,
A. Ene,
S. Escher,
S. Esen,
T. Evans,
A. Falabella,
C. F{\"a}rber,
N. Farley,
S. Farry,
D. Fazzini,
M. F{\'e}o,
P. Fernandez Declara,
A. Fernandez Prieto,
F. Ferrari,
L. Ferreira Lopes,
F. Ferreira Rodrigues,
S. Ferreres Sole,
M. Ferro-Luzzi,
S. Filippov,
R.A. Fini,
M. Fiorini,
M. Firlej,
C. Fitzpatrick,
T. Fiutowski,
F. Fleuret,
M. Fontana,
F. Fontanelli,
R. Forty,
V. Franco Lima,
M. Frank,
C. Frei,
J. Fu,
W. Funk,
E. Gabriel,
A. Gallas Torreira,
D. Galli,
S. Gallorini,
S. Gambetta,
Y. Gan,
M. Gandelman,
P. Gandini,
Y. Gao,
L.M. Garcia Martin,
J. Garc{\'\i}a Pardi{\~n}as,
B. Garcia Plana,
J. Garra Tico,
L. Garrido,
D. Gascon,
C. Gaspar,
G. Gazzoni,
D. Gerick,
E. Gersabeck,
M. Gersabeck,
T. Gershon,
D. Gerstel,
Ph. Ghez,
V. Gibson,
O.G. Girard,
P. Gironella Gironell,
L. Giubega,
K. Gizdov,
V.V. Gligorov,
C. G{\"o}bel,
D. Golubkov,
A. Golutvin,
A. Gomes,
I.V. Gorelov,
C. Gotti,
E. Govorkova,
J.P. Grabowski,
R. Graciani Diaz,
L.A. Granado Cardoso,
E. Graug{\'e}s,
E. Graverini,
G. Graziani,
A. Grecu,
R. Greim,
P. Griffith,
L. Grillo,
L. Gruber,
B.R. Gruberg Cazon,
C. Gu,
E. Gushchin,
A. Guth,
Yu. Guz,
T. Gys,
T. Hadavizadeh,
C. Hadjivasiliou,
G. Haefeli,
C. Haen,
S.C. Haines,
B. Hamilton,
X. Han,
T.H. Hancock,
S. Hansmann-Menzemer,
N. Harnew,
T. Harrison,
C. Hasse,
M. Hatch,
J. He,
M. Hecker,
K. Heinicke,
A. Heister,
K. Hennessy,
L. Henry,
M. He{\ss},
J. Heuel,
A. Hicheur,
R. Hidalgo Charman,
D. Hill,
M. Hilton,
P.H. Hopchev,
J. Hu,
W. Hu,
W. Huang,
Z.C. Huard,
W. Hulsbergen,
T. Humair,
M. Hushchyn,
D. Hutchcroft,
D. Hynds,
P. Ibis,
M. Idzik,
P. Ilten,
A. Inglessi,
A. Inyakin,
K. Ivshin,
R. Jacobsson,
S. Jakobsen,
J. Jalocha,
E. Jans,
B.K. Jashal,
A. Jawahery,
F. Jiang,
M. John,
D. Johnson,
C.R. Jones,
C. Joram,
B. Jost,
N. Jurik,
S. Kandybei,
M. Karacson,
J.M. Kariuki,
S. Karodia,
N. Kazeev,
M. Kecke,
F. Keizer,
M. Kelsey,
M. Kenzie,
T. Ketel,
B. Khanji,
A. Kharisova,
C. Khurewathanakul,
K.E. Kim,
T. Kirn,
V.S. Kirsebom,
S. Klaver,
K. Klimaszewski,
S. Koliiev,
M. Kolpin,
R. Kopecna,
P. Koppenburg,
I. Kostiuk,
S. Kotriakhova,
M. Kozeiha,
L. Kravchuk,
M. Kreps,
F. Kress,
S. Kretzschmar,
P. Krokovny,
W. Krupa,
W. Krzemien,
W. Kucewicz,
M. Kucharczyk,
V. Kudryavtsev,
G.J. Kunde,
A.K. Kuonen,
T. Kvaratskheliya,
D. Lacarrere,
G. Lafferty,
A. Lai,
D. Lancierini,
G. Lanfranchi,
C. Langenbruch,
T. Latham,
C. Lazzeroni,
R. Le Gac,
R. Lef{\`e}vre,
A. Leflat,
F. Lemaitre,
O. Leroy,
T. Lesiak,
B. Leverington,
H. Li,
P.-R. Li,
X. Li,
Y. Li,
Z. Li,
X. Liang,
T. Likhomanenko,
R. Lindner,
F. Lionetto,
V. Lisovskyi,
G. Liu,
X. Liu,
D. Loh,
A. Loi,
I. Longstaff,
J.H. Lopes,
G. Loustau,
G.H. Lovell,
D. Lucchesi,
M. Lucio Martinez,
Y. Luo,
A. Lupato,
E. Luppi,
O. Lupton,
A. Lusiani,
X. Lyu,
F. Machefert,
F. Maciuc,
V. Macko,
P. Mackowiak,
S. Maddrell-Mander,
O. Maev,
K. Maguire,
D. Maisuzenko,
M.W. Majewski,
S. Malde,
B. Malecki,
A. Malinin,
T. Maltsev,
H. Malygina,
G. Manca,
G. Mancinelli,
D. Marangotto,
J. Maratas,
J.F. Marchand,
U. Marconi,
C. Marin Benito,
M. Marinangeli,
P. Marino,
J. Marks,
P.J. Marshall,
G. Martellotti,
M. Martinelli,
D. Martinez Santos,
F. Martinez Vidal,
A. Massafferri,
M. Materok,
R. Matev,
A. Mathad,
Z. Mathe,
V. Matiunin,
C. Matteuzzi,
K.R. Mattioli,
A. Mauri,
E. Maurice,
B. Maurin,
M. McCann,
A. McNab,
R. McNulty,
J.V. Mead,
B. Meadows,
C. Meaux,
N. Meinert,
D. Melnychuk,
M. Merk,
A. Merli,
E. Michielin,
D.A. Milanes,
E. Millard,
M.-N. Minard,
O. Mineev,
L. Minzoni,
D.S. Mitzel,
A. M{\"o}dden,
A. Mogini,
R.D. Moise,
T. Momb{\"a}cher,
I.A. Monroy,
S. Monteil,
M. Morandin,
G. Morello,
M.J. Morello,
J. Moron,
A.B. Morris,
R. Mountain,
F. Muheim,
M. Mukherjee,
M. Mulder,
D. M{\"u}ller,
J. M{\"u}ller,
K. M{\"u}ller,
V. M{\"u}ller,
C.H. Murphy,
D. Murray,
P. Naik,
T. Nakada,
R. Nandakumar,
A. Nandi,
T. Nanut,
I. Nasteva,
M. Needham,
N. Neri,
S. Neubert,
N. Neufeld,
R. Newcombe,
T.D. Nguyen,
C. Nguyen-Mau,
S. Nieswand,
R. Niet,
N. Nikitin,
N.S. Nolte,
A. Oblakowska-Mucha,
V. Obraztsov,
S. Ogilvy,
D.P. O'Hanlon,
R. Oldeman,
C.J.G. Onderwater,
J. D. Osborn,
A. Ossowska,
J.M. Otalora Goicochea,
T. Ovsiannikova,
P. Owen,
A. Oyanguren,
P.R. Pais,
T. Pajero,
A. Palano,
M. Palutan,
G. Panshin,
A. Papanestis,
M. Pappagallo,
L.L. Pappalardo,
W. Parker,
C. Parkes,
G. Passaleva,
A. Pastore,
M. Patel,
C. Patrignani,
A. Pearce,
A. Pellegrino,
G. Penso,
M. Pepe Altarelli,
S. Perazzini,
D. Pereima,
P. Perret,
L. Pescatore,
K. Petridis,
A. Petrolini,
A. Petrov,
S. Petrucci,
M. Petruzzo,
B. Pietrzyk,
G. Pietrzyk,
M. Pikies,
M. Pili,
D. Pinci,
J. Pinzino,
F. Pisani,
A. Piucci,
V. Placinta,
S. Playfer,
J. Plews,
M. Plo Casasus,
F. Polci,
M. Poli Lener,
M. Poliakova,
A. Poluektov,
N. Polukhina,
I. Polyakov,
E. Polycarpo,
G.J. Pomery,
S. Ponce,
A. Popov,
D. Popov,
S. Poslavskii,
E. Price,
C. Prouve,
V. Pugatch,
A. Puig Navarro,
H. Pullen,
G. Punzi,
W. Qian,
J. Qin,
R. Quagliani,
B. Quintana,
N.V. Raab,
B. Rachwal,
J.H. Rademacker,
M. Rama,
M. Ramos Pernas,
M.S. Rangel,
F. Ratnikov,
G. Raven,
M. Ravonel Salzgeber,
M. Reboud,
F. Redi,
S. Reichert,
F. Reiss,
C. Remon Alepuz,
Z. Ren,
V. Renaudin,
S. Ricciardi,
S. Richards,
K. Rinnert,
P. Robbe,
A. Robert,
A.B. Rodrigues,
E. Rodrigues,
J.A. Rodriguez Lopez,
M. Roehrken,
S. Roiser,
A. Rollings,
V. Romanovskiy,
A. Romero Vidal,
J.D. Roth,
M. Rotondo,
M.S. Rudolph,
T. Ruf,
J. Ruiz Vidal,
J.J. Saborido Silva,
N. Sagidova,
B. Saitta,
V. Salustino Guimaraes,
C. Sanchez Gras,
C. Sanchez Mayordomo,
B. Sanmartin Sedes,
R. Santacesaria,
C. Santamarina Rios,
M. Santimaria,
E. Santovetti,
G. Sarpis,
A. Sarti,
C. Satriano,
A. Satta,
M. Saur,
D. Savrina,
S. Schael,
M. Schellenberg,
M. Schiller,
H. Schindler,
M. Schmelling,
T. Schmelzer,
B. Schmidt,
O. Schneider,
A. Schopper,
H.F. Schreiner,
M. Schubiger,
S. Schulte,
M.H. Schune,
R. Schwemmer,
B. Sciascia,
A. Sciubba,
A. Semennikov,
E.S. Sepulveda,
A. Sergi,
N. Serra,
J. Serrano,
L. Sestini,
A. Seuthe,
P. Seyfert,
M. Shapkin,
T. Shears,
L. Shekhtman,
V. Shevchenko,
E. Shmanin,
B.G. Siddi,
R. Silva Coutinho,
L. Silva de Oliveira,
G. Simi,
S. Simone,
I. Skiba,
N. Skidmore,
T. Skwarnicki,
M.W. Slater,
J.G. Smeaton,
E. Smith,
I.T. Smith,
M. Smith,
M. Soares,
l. Soares Lavra,
M.D. Sokoloff,
F.J.P. Soler,
B. Souza De Paula,
B. Spaan,
E. Spadaro Norella,
P. Spradlin,
F. Stagni,
M. Stahl,
S. Stahl,
P. Stefko,
S. Stefkova,
O. Steinkamp,
S. Stemmle,
O. Stenyakin,
M. Stepanova,
H. Stevens,
A. Stocchi,
S. Stone,
S. Stracka,
M.E. Stramaglia,
M. Straticiuc,
U. Straumann,
S. Strokov,
J. Sun,
L. Sun,
Y. Sun,
K. Swientek,
A. Szabelski,
T. Szumlak,
M. Szymanski,
Z. Tang,
T. Tekampe,
G. Tellarini,
F. Teubert,
E. Thomas,
M.J. Tilley,
V. Tisserand,
S. T'Jampens,
M. Tobin,
S. Tolk,
L. Tomassetti,
D. Tonelli,
D.Y. Tou,
R. Tourinho Jadallah Aoude,
E. Tournefier,
M. Traill,
M.T. Tran,
A. Trisovic,
A. Tsaregorodtsev,
G. Tuci,
A. Tully,
N. Tuning,
A. Ukleja,
A. Usachov,
A. Ustyuzhanin,
U. Uwer,
A. Vagner,
V. Vagnoni,
A. Valassi,
S. Valat,
G. Valenti,
M. van Beuzekom,
H. Van Hecke,
E. van Herwijnen,
C.B. Van Hulse,
J. van Tilburg,
M. van Veghel,
R. Vazquez Gomez,
P. Vazquez Regueiro,
C. V{\'a}zquez Sierra,
S. Vecchi,
J.J. Velthuis,
M. Veltri,
A. Venkateswaran,
M. Vernet,
M. Veronesi,
M. Vesterinen,
J.V. Viana Barbosa,
D. Vieira,
M. Vieites Diaz,
H. Viemann,
X. Vilasis-Cardona,
A. Vitkovskiy,
M. Vitti,
V. Volkov,
A. Vollhardt,
D. Vom Bruch,
B. Voneki,
A. Vorobyev,
V. Vorobyev,
N. Voropaev,
R. Waldi,
J. Walsh,
J. Wang,
M. Wang,
Y. Wang,
Z. Wang,
D.R. Ward,
H.M. Wark,
N.K. Watson,
D. Websdale,
A. Weiden,
C. Weisser,
M. Whitehead,
G. Wilkinson,
M. Wilkinson,
I. Williams,
M. Williams,
M.R.J. Williams,
T. Williams,
F.F. Wilson,
M. Winn,
W. Wislicki,
M. Witek,
G. Wormser,
S.A. Wotton,
K. Wyllie,
D. Xiao,
Y. Xie,
H. Xing,
A. Xu,
M. Xu,
Q. Xu,
Z. Xu,
Z. Xu,
Z. Yang,
Z. Yang,
Y. Yao,
L.E. Yeomans,
H. Yin,
J. Yu,
X. Yuan,
O. Yushchenko,
K.A. Zarebski,
M. Zavertyaev,
M. Zeng,
D. Zhang,
L. Zhang,
W.C. Zhang,
Y. Zhang,
A. Zhelezov,
Y. Zheng,
X. Zhu,
V. Zhukov,
J.B. Zonneveld,
S. Zucchelli

==> our-symbols-def.tex <==
% file for definitions that were not available in lhcb-symbols-def.tex

%%
\def\Kstars  {{\ensuremath{\kaon^{*}_0}}\xspace}
\def\Kstarsb {{\ensuremath{\Kbar{}^{*}_0}}\xspace}

\newcommand{\dif}{\ensuremath{{\rm d}}\xspace}
\newcommand{\sign}{\ensuremath{{\rm sign}}\xspace}

\newcommand{\Af}{\ensuremath{\mathcal{A}_f}\xspace}
\newcommand{\Ak}{\ensuremath{\mathcal{A}_k}\xspace}
\newcommand{\Abarf}{\ensuremath{\bar{\mathcal{A}}_f}\xspace}
\newcommand{\Abark}{\ensuremath{\bar{\mathcal{A}}_k}\xspace}
\newcommand{\Afbar}{\ensuremath{\mathcal{A}_{\bar{f}}}\xspace}
\newcommand{\Akbar}{\ensuremath{\mathcal{A}_{\bar{k}}}\xspace}
\newcommand{\Abarfbar}{\ensuremath{\bar{\mathcal{A}}_{\bar{f}}}\xspace}
\newcommand{\Abarkbar}{\ensuremath{\bar{\mathcal{A}}_{\bar{k}}}\xspace}
%% \newcommand{\CP}{\ensuremath{\mathcal{CP}}\xspace}
%% \newcommand{\CPT}{\ensuremath{\mathcal{CPT}}\xspace}
%\newcommand{\T}{\ensuremath{T}\xspace}

\def\BuToJPsiK {\decay{\Bu}{\jpsi\Kp}\xspace}

\def\BsJphi {\BsToJPsiPhi}
\def\Jmm {\jpsi(\mumu)}
\def\BsJPsimmPhi {\decay{\Bs}{\jpsi(\mumu)\phi(KK)}\xspace}
\def\BcJPsimunu {\decay{\Bc}{\Jmm \mup \Pnu}}
\newcommand{\CL}{C.L.\ }
\newcommand{\CLsb}{\ensuremath{\textrm{CL}_{\textrm{s+b}}}\xspace}
\newcommand{\CLs}{\ensuremath{\textrm{CL}_{\textrm{s}}}\xspace}
\newcommand{\CLb}{\ensuremath{\textrm{CL}_{\textrm{b}}}\xspace}
%\newcommand{\BF}{branching fraction\xspace}
\newcommand{\MC}{Monte Carlo\xspace}


\newcommand{\bb}{\ensuremath{b\bar{b}}\xspace}
\newcommand{\bbdim}{\ensuremath{b\bar{b}\to \mu \mu X}\xspace}
\newcommand{\mbdim}{\ensuremath{pp\to \mu \mu X}\xspace}
\newcommand{\Bq}{\ensuremath{B^0_q}\xspace}
%\newcommand{\Bs}{\ensuremath{B^0_s}\xspace}
%\newcommand{\Bd}{\ensuremath{B^0_d}\xspace}
%\newcommand{\Bu}{\ensuremath{B^+}\xspace}
%\newcommand{\D}{\ensuremath{D^0}\xspace}
%\newcommand{\Ks}{\ensuremath{K^0_s}\xspace}
\newcommand{\Lambdab}{\ensuremath{\Lambda^0_b}\xspace}
\newcommand{\Bsmumu}{\ensuremath{\Bs\to\mu^+\mu^-}\xspace}
\newcommand{\Bdmumu}{\ensuremath{\Bd\to\mu^+\mu^-}\xspace}
\newcommand{\KstKpi}{\ensuremath{\Kst\to K^+\pi^-}\xspace}
\newcommand{\DKpi}{\ensuremath{\D\to K^-\pi^+}\xspace}
%\newcommand{\BsKst}{\ensuremath{\Bs\to K^{*0}\bar{K^{*0}}}\xspace}
\newcommand{\Bsmumugamma}{\ensuremath{\Bs\to\mu^+\mu^-\gamma}\xspace}
\newcommand{\Bdpipi}{\ensuremath{\Bd\to\pi^+\pi^-}\xspace}
\newcommand{\Bspipi}{\ensuremath{\Bs\to\pi^+\pi^-}\xspace}
\newcommand{\BsKK}{\ensuremath{\Bs\to K^+K^-}\xspace}
\newcommand{\BdKK}{\ensuremath{\Bd\to K^+K^-}\xspace}
\newcommand{\BdKpi}{\ensuremath{\Bd\to K^+\pi^-}\xspace}
\newcommand{\BspiK}{\ensuremath{\Bs\to\pi^+K^-}\xspace}
\newcommand{\Bhh}{\ensuremath{B^0_{(s)}\to h^+h^-}\xspace}
\newcommand{\Bmm}{\ensuremath{B^0_{(s)}\to \mu^+\mu^-}\xspace}
\newcommand{\Buhhh}{\ensuremath{B^{\pm}\to h^+h^-h^{\pm}}\xspace}
\newcommand{\BsDspi}{\ensuremath{B^0_{(s)}\to  D^-_s(K^+K^-\pi^-) \pi^+}\xspace}\newcommand{\Kst}{\ensuremath{K^{*0}}\xspace}
\newcommand{\BJpsiX}{\ensuremath{B\to J/\psi X}\xspace}
\newcommand{\BuJpsiK}{\ensuremath{B^+\to J/\psi K^+}\xspace}
\newcommand{\BuJpsimumuK}{\ensuremath{B^+\to J/\psi(\mu^+\mu^-)K^+}\xspace}
\newcommand{\BJpsimumuX}{\ensuremath{B \to J/\psi(\mu^+\mu^-)X}\xspace}
\newcommand{\BdJpsiKst}{\ensuremath{B^0_d\to J/\psi K^{*0}}\xspace}
\newcommand{\BdJpsiKpi}{\ensuremath{B^0_d\to J/\psi K \pi}\xspace}
\newcommand{\BJpsiKpi}{\ensuremath{B^0_{d(s)}\to J/\psi K \pi}\xspace}
\newcommand{\BsJpsiKpi}{\ensuremath{B^0_s\to J/\psi K \pi}\xspace}
\newcommand{\BsJpsiKst}{\ensuremath{B^0_s\to J/\psi \Kstarzb}\xspace}
\newcommand{\BJpsiKst}{\ensuremath{B^0_{d(s)}\to J/\psi K^{*0}(\Kstarzb)}\xspace}
%\newcommand{\BsKstKst}{\ensuremath{B^0_s\to K^{*0}\bar{K^{*0}}}\xspace}
\newcommand{\BsKstKst}{\ensuremath{\Bs\to\Kstarz\Kstarzb}\xspace}
\newcommand{\BdKstKst}{\ensuremath{\Bd\to\Kstarz\Kstarzb}\xspace}
\newcommand{\BsKpiKpi}{\ensuremath{\Bs\to K^+\pi^-K^-\pi^+}\xspace}
\newcommand{\BdPhiKst}{\ensuremath{\Bd\to\phi\Kstarz}\xspace}
\newcommand{\BsPhiKst}{\ensuremath{\Bs\to\phi\Kstarzb}\xspace}
\newcommand{\BdRhoKst}{\ensuremath{\Bd\to\rho\Kstarzb}\xspace}
\newcommand{\BdJpsimumuKstKpi}{\ensuremath{B^0_d\to J/\psi(\mu^+\mu^-)K^{*0}(K^+\pi^-)}\xspace}
\newcommand{\BsJpsimumuKstKpi}{\ensuremath{B^0_s\to J/\psi(\mu^+\mu^-)K^{*0}(K^+\pi^-)}\xspace}
\newcommand{\BcJpsimumumunu}{\ensuremath{B^+_c\to J/\psi(\mu^+\mu^-)\mu^+\nu_{\mu}}\xspace}
\newcommand{\Jpsimumu}{\ensuremath{J/\psi\to \mu^+\mu^-}\xspace}
\newcommand{\Jpsi}{\ensuremath{J/\psi}\xspace}
\newcommand{\BdKKKpi}{\ensuremath{\Bd\to K^+ K^- K^{\pm} \pi^{\mp}}\xspace}

\newcommand{\Bqmumu}{\ensuremath{\ensuremath{B^0_{q}}\to\mu^+\mu^-}\xspace}
\newcommand{\BsJpsimumuPhiKK}{\ensuremath{B^0_s\to J/\psi(\mu^+\mu^-) \phi(K^+K^-)}\xspace}
\newcommand{\BdJpsimumupipi}{\ensuremath{B^0_d\to J/\psi(\mu^+\mu^-) \pi^+\pi^-}\xspace}
\newcommand{\BdJpsiRho}{\ensuremath{B^0_d\to J/\psi \rho^0}\xspace}
\newcommand{\BdJpsipipi}{\ensuremath{B^0_d\to J/\psi \pi^+\pi^-}\xspace}
\newcommand{\ropipi}{\ensuremath{\rho^0\to \pi^+\pi^-}\xspace}

\newcommand{\Lambdappi}{\ensuremath{\Lambda\to p\pi^-}\xspace}
\newcommand{\Lambdabppi}{\ensuremath{\Lambdab\to p\pi^-}\xspace}
\newcommand{\LambdabpK}{\ensuremath{\Lambdab\to p K^-}\xspace}
\newcommand{\Lambdabppikst}{\ensuremath{\Lambdab\to p\pi^- K^- \pi^+}\xspace}
%% \newcommand{\Lambdabppikst}{\ensuremath{\Lambdab\to p\pi^- \Kstarzb}\xspace}


\newcommand{\BsJpsiPhi}{\ensuremath{B^0_s\to J/\psi \phi}\xspace}
\newcommand{\BdRhoRho}{\ensuremath{\Bd \to \rho \rho}\xspace}

\newcommand{\BRof}[1]{\ensuremath{{\cal B}(#1)}\xspace}

\newcommand{\kkappa}{\ensuremath{K^*_0(800)}\xspace}
\newcommand{\khigh}{\ensuremath{K^*_0(1430)}\xspace}

%\newcommand{\BRof}[1]{\ensuremath{{\rm BR}(#1)}\xspace}

%\newcommand{\MeV}{\ensuremath{\,{\rm MeV}}\xspace}
%\newcommand{\GeV}{\ensuremath{\,{\rm GeV}}\xspace}
%\newcommand{\TeV}{\ensuremath{\,{\rm TeV}}\xspace}
%\newcommand{\MeVc}{\ensuremath{\,{\rm MeV}/c}\xspace}
\newcommand{\GeVc}{\ensuremath{\,{\rm GeV}/c}\xspace}
\newcommand{\MeVcc}{\ensuremath{\,{\rm MeV}/c^2}\xspace}
%\newcommand{\GeVcc}{\ensuremath{\,{\rm GeV}/c^2}\xspace}
%\newcommand{\invfb}{\ensuremath{\,{\rm fb}^{-1}}\xspace}
%\newcommand{\invpb}{\ensuremath{\,{\rm pb}^{-1}}\xspace}
%\newcommand{\invnb}{\ensuremath{\,{\rm nb}^{-1}}\xspace}
%\newcommand{\mb}{\ensuremath{\,{\rm mb}}\xspace}
\newcommand{\microb}{\ensuremath{\,{\rm \mu b}}\xspace}

\newcommand{\Enow}{\ensuremath{\,{\sqrt{s}=7\TeV}}\xspace}
\newcommand{\Einj}{\ensuremath{\,{\sqrt{s}=900\GeV}}\xspace}
\newcommand{\Enom}{\ensuremath{\,{\sqrt{s}=14\TeV}}\xspace}
\newcommand{\Efive}{\ensuremath{\,{\sqrt{s}=10\TeV}}\xspace}
\newcommand{\pdf}{\ensuremath{p.d.f.}\xspace}
\newcommand{\pdfs}{\ensuremath{p.d.f.s}\xspace}
%\newcommand{\PT}{\ensuremath{P_{\rm T}}\xspace}
%\newcommand{\ET}{\ensuremath{E_{\rm T}}\xspace}
\newcommand{\IP}{\ensuremath{{\rm IP}}\xspace}
\newcommand{\ThetaK}{\ensuremath{{\Theta_{K^{*}}}}\xspace}
\newcommand{\fdfs}{\ensuremath{\frac{f_d}{f_s}}\xspace}

%\newcommand{\IPS}{\ensuremath{{\rm IPS}}\xspace}
%\newcommand{\DOF}{\ensuremath{{\rm DOF}}\xspace}
%\newcommand{\DOFS}{\ensuremath{{\rm DOFS}}\xspace}
%\newcommand{\DOCA}{\ensuremath{{\rm DOCA}}\xspace}
%\newcommand{\DLL}{\ensuremath{{\rm \Delta LL}}\xspace}
\newcommand{\DLL}{\ensuremath{{\Delta \ln \mathcal{L}}}\xspace}
\newcommand{\gl}{\ensuremath{{\rm GL}}\xspace}
\newcommand{\glk}{\ensuremath{{\rm GL_K}}\xspace}
\newcommand{\glksm}{\ensuremath{{\rm GL_{KS}}}\xspace}
\newcommand{\glsm}{\ensuremath{{\rm GL_{S}}}\xspace}
%\newcommand{\quality}{\ensuremath{{\rm (A)}}\xspace}
%\newcommand{\noquality}{\ensuremath{{\rm (B)}}\xspace}
\newcommand{\PID}{\ensuremath{{\rm PID}}\xspace}
\newcommand{\etos}{\ensuremath{\epsilon^{TOS/SEL}}\xspace}
\newcommand{\etis}{\ensuremath{\epsilon^{TIS/SEL}}\xspace}
\newcommand{\etistos}{\ensuremath{\epsilon^{TIS\&TOS/SEL}}\xspace}

\newcommand{\etrig}{\ensuremath{\epsilon^{TRIG/SEL}}\xspace}
\newcommand{\eSelect}{\ensuremath{\epsilon^{SEL/REC}}\xspace}
\newcommand{\eReco}{\ensuremath{\epsilon^{REC}}\xspace}

\newcommand{\sumpt}{\ensuremath{{\Sigma \pt}}\xspace}
\newcommand{\maxpt}{\ensuremath{{\rm max_{\pt}}}\xspace}
\newcommand{\maxip}{\ensuremath{\rm max_{\IP}}\xspace}

\newcommand{\swave}{{S--wave}\xspace}
\newcommand{\pwave}{{P--wave}\xspace}
\newcommand{\dwave}{{D--wave}\xspace}
\newcommand{\hwave}{{H--wave}\xspace}
\newcommand{\fwave}{{F--wave}\xspace}

%\newcommand{\swave}{\ensuremath{S-wave}\xspace}
%\newcommand{\pwave}{\ensuremath{P-wave}\xspace}
%\newcommand{\dwave}{\ensuremath{D-wave}\xspace}
%\newcommand{\hwave}{\ensuremath{H-wave}\xspace}
%\newcommand{\fwave}{\ensuremath{F-wave}\xspace}


%% These commands can be placed in the preamble (to be a global definition)
%% or locally inside the \begin{table}...\end{table} syntax.
%https://www.msu.edu/~harris41/latex_tablespacing.html
\newcommand\Tstrut{\rule{0pt}{2.6ex}}
\newcommand\TTstrut{\rule{0pt}{3.2ex}}
\newcommand\Bstrut{\rule[-1.2ex]{0pt}{0pt}}
\newcommand\BBstrut{\rule[-1.8ex]{0pt}{0pt}}
\newcommand{\rhoJ}{\ensuremath{\rho_{\Jpsi}}\xspace}
\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\appref}[1]{Appendix~\ref{#1}}
\newcommand{\bibref}[1]{Ref.~\cite{#1}}
\newcommand{\secref}[1]{Sect.~\ref{#1}}
\renewcommand{\eqref}[1]{Eq.~(\ref{#1})}


\newcommand{\tred}[1]{\textcolor{red}{#1}}

\newcommand{\tabcaption}[1]{  %  for tables, so that the caption when above the float is placed correctly
\vspace{-\abovecaptionskip} % 
\caption[#1]{#1}
\vspace{\abovecaptionskip}
}

